Landau-deGennes Theory of Biaxial Nematics Re-examined

Recent experiments report that the long looked for thermotropic biaxial nematic phase has been finally detected in some thermotropic liquid crystalline systems. Inspired by these experimental observations we concentrate on some elementary theoretical issues concerned with the classical sixth-order Landau-deGennes free energy expansion in terms of the symmetric and traceless tensor order parameter $Q_{\alpha\beta}$. In particular, we fully explore the stability of the biaxial nematic phase giving analytical solutions for all distinct classes of the phase diagrams that theory allows. This includes diagrams with triple- and (tri-)critical points and with multiple (reentrant) biaxial- and uniaxial phase transitions. A brief comparison with predictions of existing molecular theories is also given.

==> COMMANDS.TEX <==
\def\btilde{\mathaccent"077E}
%
\newcommand{\bg}[1]{\mbox{\boldmath$#1$}}
\newcommand{\bll}[1]{\bf \bar{\btilde{\bg #1}}} 
\newcommand{\bfn}[1]{\mbox{\scriptsize\bf #1}}
\newcommand{\fett}[1]{% 
                        \mbox{\mathversion{bold}$#1$}}
%
\newcommand{\vecc}[1] {\stackrel{\longrightarrow}{#1}}
%
\newcommand{\examplea}{\vspace{3mm}\noindent %
                       {\sc EXAMPLE} \rule[1mm]{15.4cm}{1.5mm}\vspace{3mm} }
\newcommand{\examplesa}{\vspace{3mm}\noindent %
                      {\sc EXAMPLES} \rule[1mm]{15.15cm}{1.5mm}\vspace{3mm} }
\newcommand{\notea}{\vspace{3mm}\noindent %
                      {\sc NOTE} \rule[1mm]{16.3cm}{1.5mm} \vspace{3mm} }
\newcommand{\notesa}{\vspace{3mm} \noindent %
                      {\sc NOTES} \rule[1mm]{16.05cm}{1.5mm} \vspace{3mm} }
\newcommand{\eenda}{\vspace{3mm} \noindent  \rule[1mm]{17.6cm}{1.5mm}%
                       \vspace{3mm}}
\newcommand{\proofa}{\vspace{3mm} \noindent {\sc PROOF} %
                      \rule[1mm]{16.05cm}{1.5mm} \vspace{3mm} }
%
%
\newcommand{\exampleb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                    {\sc EXAMPLE} \rule[1mm]{15.4cm}{1.5mm}\vspace{3mm} }
\newcommand{\examplesb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                    {\sc EXAMPLES} \rule[1mm]{15.15cm}{1.5mm} \vspace{3mm} }
\newcommand{\noteb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                    {\sc NOTE} \rule[1mm]{16.3cm}{1.5mm}\vspace{3mm} }
\newcommand{\notesb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                    {\sc NOTES} \rule[1mm]{16.05cm}{1.5mm}\vspace{3mm} }
\newcommand{\eendb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                     \rule[1mm]{17.6cm}{1.5mm} \vspace{3mm} }
\newcommand{\proofb}{\vspace{3mm}\noindent\hspace{-4.6cm}%
                    {\sc PROOF} \rule[1mm]{16.05cm}{1.5mm}\vspace{3mm} }
%
%
\newcommand{\qab}{\mbox{$Q_{\alpha,\beta}({\mbox{\bf r}})$}}
%
\newcommand{\pa}{\mbox{$P_{\alpha}({\mbox{\bf r}}) $}}

